Modeling multi-legged robot locomotion with slipping and its experimental validation

Multi-legged robots with six or more legs are not in common use, despite designs with superior stability, maneuverability, and a low number of actuators being available for over 20 years. This may be in part due to the difficulty in modeling multi-legged motion with slipping and producing reliable predictions of body velocity. Here we present a detailed measurement of the foot contact forces in a hexapedal robot with multiple sliding contacts, and provide an algorithm for predicting these contact forces and the body velocity. The algorithm relies on the recently published observation that even while slipping, multi-legged robots are principally kinematic, and employ a friction law ansatz that allows us to compute the shape-change to body-velocity connection and the foot contact forces. This results in the ability to simulate motion plans for a large number of potentially slipping legs. In homogeneous environments, this can run in (parallel) logarithmic time of the planning horizon

==> experiments.tex <==
\section{Experimental setup}

\subsection{Motion capture}
We used 10 Qualisys Oqus-310+ cameras as marker-based tracking system, running at 100 fps with software QTM 2.17 build 4000. 

\subsubsection{Force/Torque measuring BigANT}
The BigANT robot has six 1 DoF legs, each actuated by a servo motor (Robotis Dynamixel MX106), via a 4-bar mechanism we chose for both foot clearance and advantageous instantaneous gearing ratios.
The detailed design and characteristics can be found in~\cite[Chapter 2.2]{zhao2021thesis}.
We manufactured the legs from foamcore (Elmer’s Products Inc. 3/8'' foam board) and fiber reinforced tape (3M Scotch \#8959) using the ``plates and reinforced flexures'' (PARF) technique of~\cite{PARF-Fitzner2017}. 
We laser-cut the base plate for the BigANT chassis from a 1/4'' ABS plastic plate. 
We then installed an 6 DoF Force/Torque sensor (ATI Gamma F/T sensor) underneath each leg, and used the vendor's wireless F/T sensor system to communicate the measurements to the controlling host computer at 100 Hz. 
We calibrated the F/T sensors according to \cite{Wu2023Calib}.

\subsubsection{Multipod robots}
We constructed the Multipod robots 3 to 6 pairs of 2-DoF segments with spring steel cantilevers as legs.
The mechanical design and characteristics can be found in~\cite[Chapter 2.3]{zhao2021thesis}.
We provide detailed documentation of the motion capture data in~\cite{Walk_slither_Zhao2022}, and the dataset itself can be found in~\cite{Multipod-processed-data, Multipod-raw-data, Multipod-raw-videos}.
To model the body motion of unloaded spring legs, we computed the location of each foot relative to the rigid segment to which its spring was connected using motion tracking frames in which the leg was unloaded.
We then extrapolated this unloaded position to the frames where the leg was loaded.

\subsubsection{Ghost Robotics Spirit}
We used a Spirit 40 v1.0 Proto Q-UGV Robot from Ghost robotics, operated through a Samsung Galaxy A50 with on board firmware version 0.12.6.

\subsection{Parameter fitting of $K$, $\mu$ and $\HT$}
We estimated the spring constants $K$ by minimizing the L2-norm difference between modeled and measured $\zOf{F}{}$ distribution among contacting legs, while adding the coefficient of variation of $K$ between legs as a regularization penalty.
We assumed anisotropic friction coefficients $\HT_k$ (see \refEqn{anisotropic}), and inferred the parameters $\mu_k$ and $\xyOf{\w}{k}$ for each leg by minimizing L2-norm error between measured forces and forces calculated from slipping velocity measured by motion capture.
We used \texttt{scipy.optimize.least\_squares} for both of these parameter estimation minimizations.

We solved for classical Coulomb friction with \texttt{scipy.optimize.root} using the LM algorithm, with the solution of the previous time-step as an initial guess.
Because Coulomb friction is non-smooth, we approximated the solution starting from $\varepsilon=10^{-5}$ (from \refEqn{h2}), using each solution as an initial condition for another solution with smaller $\varepsilon$ until the relative change in L2-norm of two consecutive solutions differed less than $10^{-3}$ -- a threshold less than $5\%$ of the median ground speed measured.
In the very rare cases (0.12\% of the BigANT tripod gait dataset) where the Coulomb friction solver failed to converge, we used the ground truth velocity as the initial condition to obtain the Coulomb friction solution, and these converged.


